FreshVLA: Frequency-Regularized Time Scale Hierarchical Latent Actions for Vision-Language-Action Models

Learning reusable latent actions from action-free videos offers an effective route to improving Vision-Language-Action (VLA) policies. However, reconstruction-oriented latent actions do not necessarily benefit policy learning: as they may encode task-irrelevant static appearance with scene identity, or entangle slowly varying task progress with fine-grained execution dynamics in limited discrete code. We propose FreshVLA, a VLA framework built on a frequency-guided, dynamics-sensitive learning paradigm for acquiring temporally hierarchical continuous latent actions. FreshVLA uses a high-pass prior to guide visual transition encoding toward dynamical regions, thereby reducing reliance on static appearance cues. It further organizes latent actions into coarse-grained task progress and fine-grained execution dynamics through cross-timescale sampling and frequency-domain regularization, enhancing their capacity to represent long-horizon behaviors. During policy training, we freeze the pretrained latent action encoder and transfer its representations to robot control through joint flow-matching of latent and robot actions. FreshVLA achieves 98.2% average success on LIBERO and 98.0% on LIBERO-Long, exceeding GR00T-N1.6 on the latter by 3.6%. It also reaches an average sequence length of 4.52 on CALVIN and strong overall success rate of 80.4% in the zero-shot LIBERO-PLUS evaluation. Furthermore, FreshVLA exhibits greater robustness to visual perturbations and a more distinct division of roles between two branches in modeling low- and high-frequency motion, respectively. In 35-step action regression, it achieves a 51.3-percentage-point higher relative error reduction than its hierarchical discrete counterpart. Real-world experiments demonstrate that FreshVLA improves the average success rate over $\pi_{0.5}$ by 7.5%. The FreshVLA project page is available at https://freshvla.github.io/.

==> frame-06.tex <==
\definecolor{edgeink}{HTML}{337B80}\definecolor{edgerule}{HTML}{41888B}
\makeatletter
\patchcmd{\sa@maketitle@fancy}{colframe=titleframe,}{colframe=white,overlay={\draw[edgeink,rounded corners=4pt,line width=.45pt] ([shift={(2pt,2pt)}]frame.south west) rectangle ([shift={(-2pt,-2pt)}]frame.north east); \draw[edgeink,line width=2pt] ([shift={(2pt,-17pt)}]frame.north west)--([shift={(2pt,-2pt)}]frame.north west)--++(16pt,0); \draw[edgeink,line width=2pt] ([shift={(-18pt,2pt)}]frame.south east)--++(16pt,0)--++(0,15pt);},}{}{\PackageError{cover}{Frame patch failed}{}}
\renewcommand{\sa@fancydivider}{\noindent\begin{tikzpicture}\useasboundingbox (0,-1pt) rectangle (\linewidth,2pt);\draw[edgerule,line width=.5pt] (0,0)--(\linewidth,0);\draw[edgerule,line width=1.8pt] (0,0)--(18pt,0);\end{tikzpicture}\par\vspace{-\parskip}}
\makeatother
